Preserving Linear Separability in Continual Learning by Backward Feature Projection

Catastrophic forgetting has been a major challenge in continual learning, where the model needs to learn new tasks with limited or no access to data from previously seen tasks. To tackle this challenge, methods based on knowledge distillation in feature space have been proposed and shown to reduce forgetting. However, most feature distillation methods directly constrain the new features to match the old ones, overlooking the need for plasticity. To achieve a better stability-plasticity trade-off, we propose Backward Feature Projection (BFP), a method for continual learning that allows the new features to change up to a learnable linear transformation of the old features. BFP preserves the linear separability of the old classes while allowing the emergence of new feature directions to accommodate new classes. BFP can be integrated with existing experience replay methods and boost performance by a significant margin. We also demonstrate that BFP helps learn a better representation space, in which linear separability is well preserved during continual learning and linear probing achieves high classification accuracy. The code can be found at https://github.com/rvl-lab-utoronto/BFP

==> fig-relacc-old.tex <==
\begin{figure}[!t]
    \centering
    % \includegraphics[width=\linewidth]{figures/rel-acc.pdf}
    \includegraphics[width=\linewidth]{figures/cifar100-svd.pdf}
    \includegraphics[width=\linewidth]{figures/cifar100-svd-rel.pdf}
    \includegraphics[width=\linewidth]{figures/cifar100-acc.pdf}
    \includegraphics[width=\linewidth]{figures/cifar100-acc-rel.pdf}
    \caption{
    % \qiao{Note two plots show absolute values and the other two show relative values. We should select absolute or the relative ones. Please see which ones are better. }
    % Accuracies quickly saturate when only a small subspace in feature space is kept for incremental classification task. Here each curve shows the relative accuracy (w.r.t. using full feature space) versus the number of dimensions kept. 
    Feature distribution and importance for classification using an oracle CL method (JT) and a naive one (FT). Upper plot: feature variance (singular values) along each principal direction. Lower plot: classification accuracies using features that are projected on a subspace formed by $k$ principal vectors (note that the right endpoint of all curves already, saturates, achieving more than 99\% of the full accuracy). Different curves are obtained at the end of different tasks during continual learning, and the legend shows how many classes have been seen so far. As the model is trained on more classes, more feature dimensions are used for classification, but still remain a small portion compared to the full feature dimension (512). 
    \qiao{Are second and fourth plot better? - Make it a 2x2 grid of plots. }
    }
    \label{fig:relacc}
\end{figure}

